Hopf dreams and diagonal harmonics

This paper introduces a Hopf algebra structure on a family of reduced pipe dreams. We show that this Hopf algebra is free and cofree, and construct a surjection onto a commutative Hopf algebra of permutations. The pipe dream Hopf algebra contains Hopf subalgebras with interesting sets of generators and Hilbert series related to subsequences of Catalan numbers. Three other relevant Hopf subalgebras include the Loday-Ronco Hopf algebra on complete binary trees, a Hopf algebra related to a special family of lattice walks on the quarter plane, and a Hopf algebra on $\nu$-trees related to $\nu$-Tamari lattices. One of this Hopf subalgebras motivates a new notion of Hopf chains in the Tamari lattice, which are used to present applications and conjectures in the theory of multivariate diagonal harmonics.

==> figures/dominantPipeDreamsPacking1.tex <==
$
\pipeDreamBiColor{blue, dashed}{red}{black}{
	{n,n,\b{6},\b{5},\b{7},\b{4},\r{2},\r{1},\r{3}},
	{n,e/b/r,c/r/l,c/r/l,c/r/l,c/r/l,e/r/r,e/r/r,e/r/b},
	{\r{1},c/r/r,c/r/l,c/r/l,c/r/l,c/r/l,e/r/r,e/r/b},
	{\r{2},e/r/l,c/l/l,e/l/r,c/r/l,c/r/l,e/r/b},
	{\r{3},c/r/l,c/r/l,e/r/l,c/l/l,e/l/b},
	{\b{4},c/l/l,c/l/l,e/l/l,e/l/b},
	{\b{5},e/l/l,e/l/l,e/l/b},
	{\b{6},e/l/l,e/l/b},
	{\b{7},e/l/b},
}
$

==> figures/dominantPipeDreamsPacking2.tex <==
$
\pipeDreamMonoColor{blue, dashed}{black}{
	{n,n,\b{6},\b{5},\b{7},\b{4}},
	{n,t,c,e,c,b},
	{\b{4},c,c,e,b},
	{\b{5},e,e,b},
	{\b{6},e,b},
	{\b{7},b},
}
$

==> figures/dominantPipeDreamsPacking3.tex <==
$
\pipeDreamMonoColor{red}{black}{
	{n,n,\r{2},\r{1},\r{3}},
	{n,t,e,e,b},
	{\r{1},c,e,b},
	{\r{2},e,b},
	{\r{3},b},
}
$

==> figures/flipPipeDreams.tex <==
\begin{figure}[h]
	\centerline{
		\pipeDreamMonoColor{black}{black}{
			{n,n,1,5,4,2,3},
			{n,t,e,e,c,e,b},
			{1,e,e,e,c,b},
			{2,c,e,e,b},
			{3,c,e,b},
			{4,c,b},
			{5,b},
		}
		\quad
		\pipeDreamMonoColor{black}{black}{
			{n,n,1,5,4,2,3},
			{n,t,e,e,c,e,b},
			{1,e,e,e,e,b},
			{2,c,e,e,b},
			{3,c,c,b},
			{4,c,b},
			{5,b},
		}
	}
	\caption{Two pipe dreams of~$\pipeDreams_5$ connected by a flip.}
	\label{fig:flipPipeDreams}
\end{figure}

==> figures/horizontalPackingPipeDreamBis.tex <==
$
\r{\lrot_2(P)}
\left(\raisebox{.2cm}{
\pipeDreamBiColor{blue, dashed}{red}{black}{
	{n,n,\b{6},\b{3},\b{5},\b{4},\r{2},\r{1}},
	{n,e/r/l,e/l/l,e/l/r,c/r/l,c/r/l,e/r/r,e/r/b},
	{\r{1},c/r/l,c/r/l,c/r/r,c/r/l,c/r/l,e/r/b},
	{\r{2},c/r/l,c/r/l,e/r/l,e/l/l,e/l/b},
	{\b{3},c/l/l,e/l/l,e/l/l,e/l/b},
	{\b{4},c/l/l,c/l/l,e/l/b},
	{\b{5},c/l/l,e/l/b},
	{\b{6},e/l/b},
}
}\right)
=
\pipeDreamBiColorHorizontalPacking{blue}{red}{black}{
	{n,n,n,n,n,n,\r{2},\r{1}},
	{n,e/r/l,n,e/l/r,h/r/l,h/r/l,e/r/r,e/r/b},
	{\r{1},h/r/l,h/r/l,c/r/r,h/r/l,h/r/l,e/r/b},
	{\r{2},h/r/l,h/r/l,e/r/l,n,n},
}
=
\pipeDreamMonoColor{red}{black}{
	{n,n,\r{2},\r{1}},
	{n,t,e,b},
	{\r{1},c,b},
	{\r{2},b},
}
$

==> figures/nonAssociative.tex <==
\begin{figure}[h]
	\centerline{$\begin{array}{ccl}
		\left(
		\pipeDreamMonoColor{blue}{black}{
			{tb,t,b},
			{t,b},
			{b},
		}	
		\product
		\pipeDreamMonoColor{red}{black}{
			{tb,t,b},
			{t,b},
			{b},
		}	
		\right)
		\product
		\pipeDreamMonoColor{darkgreen}{black}{
			{tb,t,b},
			{t,b},
			{b},
		}	
		& = &
		\pipeDreamTriColor{blue}{red}{darkgreen}{black}{
			{e/b/b,e/b/l,c/l/r,c/l/m,e/l/b},
			{e/b/l,e/l/m,c/m/r,e/m/b},
			{e/l/m,e/m/r,e/r/b},
			{e/m/r,e/r/b},
			{e/r/b},
		}
		\,+\,
		\pipeDreamTriColor{blue}{red}{darkgreen}{black}{
			{e/b/b,e/b/l,c/l/m,c/l/r,e/l/b},
			{e/b/l,e/l/m,e/m/r,e/r/b},
			{e/l/m,e/m/r,e/r/b},
			{c/r/m,e/r/b},
			{e/m/b},
		}
		\,+\,
		\pipeDreamTriColor{blue}{red}{darkgreen}{black}{
			{e/b/b,e/b/l,e/l/m,c/m/r,e/m/b},
			{e/b/l,e/l/m,e/m/r,e/r/b},
			{c/m/l,e/m/r,e/r/b},
			{c/r/l,e/r/b},
			{e/l/b},
		}
		\,+\,
		\pipeDreamTriColor{blue}{red}{darkgreen}{black}{
			{e/b/b,e/b/l,e/l/m,e/m/r,e/r/b},
			{e/b/l,e/l/m,e/m/r,e/r/b},
			{c/r/l,c/r/m,e/r/b},
			{c/m/l,e/m/b},
			{e/l/b},
		}
		\,+\,
		\pipeDreamTriColor{blue}{red}{darkgreen}{black}{
			{e/b/b,e/b/l,c/l/m,e/l/r,e/r/b},
			{e/b/l,e/l/m,e/m/r,e/r/b},
			{c/r/l,c/r/m,e/r/b},
			{e/l/m,e/m/b},
			{e/m/b},
		}
		\,+\,
		\pipeDreamTriColor{blue}{red}{darkgreen}{black}{
			{e/b/b,e/b/l,c/l/r,e/l/m,e/m/b},
			{e/b/l,e/l/m,c/m/r,e/m/b},
			{c/m/l,e/m/r,e/r/b},
			{e/l/r,e/r/b},
			{e/r/b},
		}
		\\
		\\
%		& = &
%		\pipeDreamMonoColor{blue}{black}{
%			{tb,t,b},
%			{t,b},
%			{b},
%		}	
%		\product
%		\left(
%		\pipeDreamMonoColor{red}{black}{
%			{tb,t,b},
%			{t,b},
%			{b},
%		}	
%		\product
%		\pipeDreamMonoColor{darkgreen}{black}{
%			{tb,t,b},
%			{t,b},
%			{b},
%		}	
%		\right)
%		\,+\,
%		\pipeDreamTriColor{blue}{red}{darkgreen}{black}{
%			{e/b/b,e/b/l,c/l/m,e/l/r,e/r/b},
%			{e/b/l,e/l/m,e/m/r,e/r/b},
%			{c/r/l,c/r/m,e/r/b},
%			{e/l/m,e/m/b},
%			{e/m/b},
%		}
%		\,+\,
%		\pipeDreamTriColor{blue}{red}{darkgreen}{black}{
%			{e/b/b,e/b/l,c/l/r,e/l/m,e/m/b},
%			{e/b/l,e/l/m,c/m/r,e/m/b},
%			{c/m/l,e/m/r,e/r/b},
%			{e/l/r,e/r/b},
%			{e/r/b},
%		}
		\pipeDreamMonoColor{blue}{black}{
			{tb,t,b},
			{t,b},
			{b},
		}	
		\product
		\left(
		\pipeDreamMonoColor{red}{black}{
			{tb,t,b},
			{t,b},
			{b},
		}	
		\product
		\pipeDreamMonoColor{darkgreen}{black}{
			{tb,t,b},
			{t,b},
			{b},
		}	
		\right)
		& = &
		\pipeDreamTriColor{blue}{red}{darkgreen}{black}{
			{e/b/b,e/b/l,c/l/r,c/l/m,e/l/b},
			{e/b/l,e/l/m,c/m/r,e/m/b},
			{e/l/m,e/m/r,e/r/b},
			{e/m/r,e/r/b},
			{e/r/b},
		}
		\,+\,
		\pipeDreamTriColor{blue}{red}{darkgreen}{black}{
			{e/b/b,e/b/l,c/l/m,c/l/r,e/l/b},
			{e/b/l,e/l/m,e/m/r,e/r/b},
			{e/l/m,e/m/r,e/r/b},
			{c/r/m,e/r/b},
			{e/m/b},
		}
		\,+\,
		\pipeDreamTriColor{blue}{red}{darkgreen}{black}{
			{e/b/b,e/b/l,e/l/m,c/m/r,e/m/b},
			{e/b/l,e/l/m,e/m/r,e/r/b},
			{c/m/l,e/m/r,e/r/b},
			{c/r/l,e/r/b},
			{e/l/b},
		}
		\,+\,
		\pipeDreamTriColor{blue}{red}{darkgreen}{black}{
			{e/b/b,e/b/l,e/l/m,e/m/r,e/r/b},
			{e/b/l,e/l/m,e/m/r,e/r/b},
			{c/r/l,c/r/m,e/r/b},
			{c/m/l,e/m/b},
			{e/l/b},
		}
	\end{array}$}
	\caption{The product on pipe dreams is not associative.}
	\label{fig:productPipeDreamsNonAssociative}
\end{figure}


==> figures/productPipeDreamsCambrian.tex <==
\begin{figure}[h]
	\centerline{$
		\pipeDreamMonoColor{blue}{black}{
			{n,n,n,n,t,c},
			{n,n,n,t,e,c,c,c,c},
			{n,n,t,c,e,e,c,c,c},
			{n,t,e,c,c,e,e,c,b},
			{t,c,e,e,c,c,e,b},
			{n,n,c,e,e,c,b},
			{n,n,c,c,e,b},
			{n,n,c,c,b},
			{n,n,n,b},
		}
		\star_{\b{p}\r{qq}\b{p}\r{qq}\b{ppp}\r{q}\b{p}\r{qq}\b{p}\r{q}} \;
		\pipeDreamMonoColor{red}{black}{
			{n,n,n,n,n,t},
			{n,n,n,n,t,e},
			{n,n,n,t,e,e,e,c,c},
			{n,n,t,c,e,c,e,c,c},
			{n,t,c,c,e,c,e,c,c,b},
			{t,c,c,c,e,e,e,e,b},
			{c,c,c,c,c,e,c,b},
			{n,n,c,c,c,e,b},
			{n,n,c,c,c,b},
			{n,n,c,c,b},
		}
		=
		\pipeDreamBiColor{blue}{red}{black}{
			{n,n,n,n,n,n,n,n,e/b/l,e/l/r},
			{n,n,n,n,n,n,n,e/b/l,e/l/r,e/r/r},
			{n,n,n,n,n,n,e/b/l,c/l/l,c/l/r,c/l/r},
			{n,n,n,n,n,e/b/l,e/l/l,c/l/l,c/l/r,c/l/r,c/l/r,c/l/r,c/l/l,c/l/l,c/l/l,c/l/r},
			{n,n,n,n,e/b/l,c/l/l,e/l/l,c/l/l,c/l/r,c/l/r,c/l/r,c/l/r,e/l/l,c/l/l,e/l/r,c/r/r},
			{n,n,n,e/b/l,e/l/l,e/l/l,c/l/l,c/l/l,c/l/r,c/l/r,c/l/r,c/l/r,e/l/l,e/l/r,e/r/r,c/r/r},
			{n,n,e/b/l,c/l/l,c/l/l,c/l/l,c/l/l,c/l/l,c/l/r,c/l/r,c/l/r,c/l/r,c/l/l,c/l/r,c/l/r,c/l/r},
			{n,e/b/l,e/l/r,c/r/l,c/r/l,c/r/l,c/r/l,c/r/l,c/r/r,c/r/r,c/r/r,c/r/r,c/r/l,e/r/r,e/r/r,c/r/r,e/r/b},
			{e/b/l,e/l/r,c/r/r,c/r/l,c/r/l,c/r/l,c/r/l,c/r/l,c/r/r,c/r/r,c/r/r,c/r/r,c/r/l,e/r/r,e/r/r,e/r/b},
			{c/r/l,c/r/r,c/r/r,c/r/l,c/r/l,c/r/l,c/r/l,c/r/l,c/r/r,c/r/r,c/r/r,c/r/r,c/r/l,e/r/r,e/r/b},
			{n,n,n,n,c/r/l,c/r/l,c/r/l,c/r/l,c/r/r,c/r/r,c/r/r,c/r/r,c/r/l,e/r/b},
			{n,n,n,n,c/l/l,e/l/l,c/l/l,c/l/l,c/l/r,c/l/r,c/l/r,c/l/r,e/l/b},
			{n,n,n,n,c/l/l,e/l/l,e/l/r,c/r/l,e/r/r,e/r/r,e/r/r,e/r/b},
			{n,n,n,n,c/l/l,e/l/r,c/r/r,c/r/l,e/r/r,c/r/r,e/r/b},
			{n,n,n,n,c/r/l,c/r/r,c/r/r,c/r/l,e/r/r,e/r/b},
			{n,n,n,n,c/r/l,c/r/r,c/r/r,c/r/l,e/r/b},
			{n,n,n,n,n,n,n,e/l/b},
		}
	$}
	\caption{Two pipe dreams on tiling shapes (left), and an element in their product (right).}
	\label{fig:productPipeDreamsCambrian}
\end{figure}

==> figures/reversingPipeDreamsDepthZero.tex <==
\begin{figure}[h]
	\centerline{
		\pipeDreamMonoColor{black}{black}{
			{b},
		}
		\quad
		\pipeDreamMonoColor{black}{black}{
			{c,b},
			{b},
		}
		\quad
		\pipeDreamMonoColor{black}{black}{
			{c,c,b},
			{c,b},
			{b},
		}
		\quad
		\pipeDreamMonoColor{black}{black}{
			{c,c,c,b},
			{c,c,b},
			{c,b},
			{b},
		}
		\quad
		\pipeDreamMonoColor{black}{black}{
			{c,c,c,c,b},
			{c,c,c,b},
			{c,c,b},
			{c,b},
			{b},
		}
		\quad
		\pipeDreamMonoColor{black}{black}{
			{c,c,c,c,c,b},
			{c,c,c,c,b},
			{c,c,c,b},
			{c,c,b},
			{c,b},
			{b},
		}
		\quad
		\pipeDreamMonoColor{black}{black}{
			{c,c,c,c,c,c,b},
			{c,c,c,c,c,b},
			{c,c,c,c,b},
			{c,c,c,b},
			{c,c,b},
			{c,b},
			{b},
		}
	}
	\caption{The pipe dreams~$P^{[n]}$ for~$n \in [7]$.}
	\label{fig:reversingPipeDreamsDepthZero}
\end{figure}

==> figures/untanglePipeDreamBis.tex <==
$
\coproduct_{4,2}\left(\raisebox{.2cm}{
\pipeDreamBiColor{blue, dashed}{red}{black}{
	{n,n,\b{6},\b{3},\b{5},\b{4},\r{2},\r{1}},
	{n,e/b/l,e/l/l,e/l/r,c/r/l,c/r/l,e/r/r,e/r/b},
	{\r{1},c/r/l,c/r/l,c/r/r,c/r/l,c/r/l,e/r/b},
	{\r{2},c/r/l,c/r/l,e/r/l,e/l/l,e/l/b},
	{\b{3},c/l/l,e/l/l,e/l/l,e/l/b},
	{\b{4},c/l/l,c/l/l,e/l/b},
	{\b{5},c/l/l,e/l/b},
	{\b{6},e/l/b},
}
}\right)
=
\pipeDreamMonoColor{blue, dashed}{black}{
	{n,n,\b{4},\b{1},\b{3},\b{2}},
	{n,t,e,e,e,b},
	{\b{1},c,e,e,b},
	{\b{2},c,c,b},
	{\b{3},c,b},
	{\b{4},b},
}
\otimes
\pipeDreamMonoColor{red}{black}{
	{n,n,\r{2},\r{1}},
	{n,t,e,b},
	{\r{1},c,b},
	{\r{2},b},
}
$
